ISAC MIMO Systems with OTFS Waveforms and Virtual Arrays

A novel Integrated Sensing-Communication (ISAC) system is proposed that can accommodate high mobility scenarios while making efficient use of bandwidth for both communication and sensing. The system comprises a monostatic multiple-input multiple-output (MIMO) radar that transmits orthogonal time frequency space (OTFS) waveforms. Bandwidth efficiency is achieved by making Doppler-delay (DD) domain bins available for shared use by the transmit antennas. For maximum communication rate, all DD-domain bins are used as shared, but in this case, the target resolution is limited by the aperture of the receive array. A low-complexity method is proposed for obtaining coarse estimates of the radar targets parameters in that case. A novel approach is also proposed to construct a virtual array (VA) for achieving a target resolution higher than that allowed by the receive array. The VA is formed by enforcing zeros on certain time-frequency (TF) domain bins, thereby creating private bins assigned to specific transmit antennas. The TF signals received on these private bins are orthogonal, enabling the synthesis of a VA. When combined with coarse target estimates, this approach provides high-accuracy target estimation. To preserve DD-domain information, the introduction of private bins requires reducing the number of DD-domain symbols, resulting in a trade-off between communication rate and sensing performance. However, even a small number of private bins is sufficient to achieve significant sensing gains with minimal communication rate loss. The proposed system is robust to Doppler frequency shifts that arise in high mobility scenarios.

==> 02model.tex <==
% We assume a monostatic MIMO radar  with $N_t$ transmit antennas and $N_r$ receive antennas operating at carrier frequency $f_c$ Hz. The radar transmits an OTFS waveform carrying information for a communication receiver.%  \textcolor{red}{I think here you just have the OTFS background and $J$ is not the number of targets but the number of obstacles in the path of the communication signal (some of those will create reflections back to the radar but not all of them}
% \textcolor{green}{I think we can define $J$ is the number of paths in the channel. In radar the paths are backscatter from targets, and in communication the paths are obstacles in the environments. With this justification we can save some parameters..}
% There are $J$ targets that reflect the transmitted signal. Based on the received target echoes the radar will detect the presence of targets and estimates their  range, velocity, and angle.% The channel \textcolor{red}{the channel between what points???} is modeled as a $J$-tap doubly-selective channel in the DD domain~\cite{8424569}
% \begin{align}
%     \label{eq:DDChannel}
%     h(\nu,\tau)=\sum_{j=0}^{J-1}\beta_j \delta(\nu-\nu_j)\delta(\tau-\tau_j),
% \end{align}
% \textcolor{red}{what about the channel to the communication receiver?}
% where $J$ is the number of targets, $\nu_j=\frac{2v_jf_c}{c}$ is the round-trip Doppler shift caused by the $j$-th target moving at speed $v_j$, $c$ is the speed of light, $\tau_j=\frac{2R_j}{c}$ is the round-trip delay of the $j$-th target at range $R_j$, and $\beta_j$ is the channel gain.
% We denote $\lambda=\frac{c}{f_c}$ as the radar wavelength.
% % Hence, the time-frequency domain channel gain is $\beta_je^{-j2\pi\nu_j\tau_j}$.% \subsection{OTFS Modulation and Demodulation}\label{sec:demodulation}
In this section, we introduce OTFS waveforms in the context of a SISO communication system.

The system transmits packet bursts, each of duration $T=N\Delta t$ with bandwidth $B=M\Delta f$, where $N$ is the number of subsymbols, $M$ is the number of subcarriers, $\Delta t$ is the subsymbol duration, and $\Delta f$ is the subcarrier spacing.
The orthogonality condition requires that $\Delta t \cdot \Delta f = 1$~\cite{mohammed2020derivation}.
In each burst, a set of $NM$ complex information-bearing symbols are arranged on the DD grid,
\begin{align*}
   \set{\parens*{k\Delta \nu, l\Delta\tau} \mid k=0,1,\ldots,N-1;l=0,1,\ldots,M-1},
\end{align*}
where $k$ and $l$ are Doppler and delay indices, and
the grid spacing is
\begin{align}
    \Delta \nu&={1}/({N\Delta t}) & \Delta \tau &={1}/({M\Delta f}). & \label{eq:DD_spacing}
\end{align}
The transmitted signal is reflected by $J$ point reflectors, each introducing a Doppler and delay that are multiples of the corresponding grid spacing, \ie
\begin{align}
    \nu_{j}&=(k_{j}+\kappa_{j})\Delta\nu, &k_{j}&\in\Z, &\kappa_{j}&\in\bracks*{-0.5,0.5},& \label{eq:Doppler_spacing}\\
    \tau_{j}&=(l_{j}+\iota_{j})\Delta\tau, &l_{j}&\in\Z^{+}, &\iota_{j}&\in\bracks*{-0.5,0.5}.& \label{eq:Delay_spacing}
\end{align}
% $\nu_j=(k_{j}+\kappa_{j})\Delta\nu$,
% $k_{j}\in\Z$, $\kappa_{j}\in\bracks*{-0.5,0.5}$,
% and $\tau_j=(l_{j}+\iota_{j})\Delta\tau$, $l_{j}\in\Z^{+}$, $\iota_{j}\in\bracks*{-0.5,0.5}$.
The dimensions of the grid
%satisfy $N\geq 2\max \abs{k_{\nu_j}}$ and $M\geq\max l_{\tau_j}$ so
are such that can support all present Doppler and delays.
The complex gain introduced by each reflector is $\beta_j$.
The presence of $\kappa_{j}$ and $\iota_{j}$ are known as fractional Doppler and fractional Delay, respectively.
The $\kappa_{j}$ and $\iota_{j}$ vanish quickly as $\Delta\nu$ and $\Delta\tau$ become finer, \ie increasing $N$ and $M$ for the same symbol duration $T$ and bandwidth $B$.
Modern communication systems tend to synthesize a wide-band waveform with multiple narrow-band signals, and hence, it is safe to assume $\iota_{j}\rightarrow0$ with a preferred large $M$.
However, $N$ is usually small for low-latency communication, and $\kappa_{j}$ is generally present.
% \textcolor{green}{We need to define $\nu_j$ and $\tau_j$}

The OTFS transmitter maps the information-bearing symbol placed on the DD grid, \ie $x[k,l]$,
% (denoted as $X_{DD}[l+kM]$)
to the TF grid, \ie $X[n,m]$, via the Inverse Symplectic Finite Fourier Transform (ISFFT)~\cite{ronny2017otfs},
% (\ie $X_{TF}[m+nM]$ for TF bin $[n, m]$),
% \footnote{The ISFFT is $N$-point DFT along the time\textcol or{blue}{/Doppler} axis and the $M$-point IDFT along the frequency\textcolor{blue}{/delay} axis.}
\begin{align}\label{eq:ISFFT}
    X[n,m] = \frac{1}{NM}\sum_{k=0}^{N-1}\sum_{l=0}^{M-1}x[k,l]e^{j2\pi\parens*{\frac{kn}{N}-\frac{ml}{M}}}.
\end{align}
The analog signal for transmission, $s(t)$, is created via the  Heisenberg Transform~\cite{ronny2017otfs}, \ie
\begin{align}\label{eq:Heisenberg}
    s(t) = \sum_{n=0}^{N-1}\sum_{m=0}^{M-1}X[n,m]g_{tx}(t-n\Delta t)e^{j2\pi m\Delta f(t-n\Delta t)},
\end{align}
where $g_{tx}(t)$ is the pulse function of the transmitter.
% In the rest of the paper, we assume all pulse functions are a rectangular pulse.
The baseband signal, $s^{k,l}(t)$, corresponding to $x[k,l]$ is~\cite{UbadahZakOTFS}
% \textcolor{blue}{\cite[eq 103]{UbadahZakOTFS}. It is $\delta$ for the case of infinity bandwidth and $\sinc$ for realistic bandlimited signal. Can also be seen from~\cite[eq 14 15]{mohammed2020derivation}}
% \textcolor{purple}{\Cref{eq:ISFFT} is $\mathbf{X}=(\mathbf{F}_N^H \otimes \mathbf{F}_M) \mathbf{x}$. \Cref{eq:Heisenberg} is $s(t)=(\mathbf{G}_{tx}\otimes \mathbf{F}_M^H)\mathbf{X}$. Then~\cref{eq:baseband} is $s(t)=(\mathbf{G}_{tx}\otimes \mathbf{F}_M^H)(\mathbf{F}_N^H \otimes \mathbf{F}_M) \mathbf{x}=(\mathbf{G}_{tx}\otimes \mathbf{F}_N^H)\mathbf{x}$. Then $g_{tx}$ is $\delta$ for ideal case or $\sinc$ for bandlimited case in~\cref{eq:baseband}. The $e^{j2\pi\frac{nk}{N}}$ is the realization of $\mathbf{F}_N^H$. Maybe I should just use $g_{tx}$.}
\begin{align}\label{eq:baseband}
    s^{k,l}(t)=\sum_{n=0}^{N-1}x[k,l]e^{j2\pi\frac{nk}{N}}g_{tx}\parens*{t-n\Delta t-\frac{l}{M}\Delta t}.
\end{align}
% and can be viewed as the Zak Transform of $d[l+kM]$, which is a composition of an ISFFT and a Heisenberg Transform.
Omitting noise, the analog received signal is
\begin{align}\label{eq:received}
    r(t)=\sum_{j=0}^{J-1} \beta_j s(t-\tau_j)e^{j2\pi\nu_j (t-\tau_j)}.
\end{align}
At the receiver, upon matched filtering and sampling
% a matched filter computes the cross-ambiguity $A_{g_{rx},y}(t,f)$ between received signals $y(t)$ and the receiver pulse function $g_{rx}(t)$,
% \begin{align}
%     \label{eq:CAF}
%     Y(t,f)=A_{g_{rx},y}(t,f)\stackrel{\Delta}{=}\int y(t')g_{rx}\!^*(t'-t)e^{-j2\pi f(t'-t)}\diff t'.\notag
% \end{align}
% By sampling $Y(t,f)$
for a duration $T$ at frequency $B$ with receiver pulse function $g_{rx}(t)$ (\aka Wigner Transform~\cite{ronny2017otfs}), the TF domain samples $Y[n,m]$ are obtained.
Assuming that $g_{tx}$, $g_{rx}$ are bi-orthogonal, it holds that
\begin{align}
    Y[n,m]
    &=X[n,m]H[n,m], \label{eq:TFIO} \\
    H[n,m]
    &=\sum_{j=0}^{J-1} \beta_j e^{-j2\pi\nu_j\tau_j} e^{j2\pi(\nu_j n\Delta t-m\Delta f\tau_j)}. \label{eq:TFChannel}
\end{align}
% }%
% where $H$ is the effective time-frequency channel~\cite{ronny2017otfs,8424569,wei2020transmitterreceiverwindowdesigns}.
% \textcolor{red}{This sections about communication system. Explain how the transmitted symbols can be receiver at the receiver. *********}
% where $H_{n,m}$ is the time-frequency channel.
% $H$ can be viewed as the circular convolution of the ISFFT of~\cref{eq:DDChannel} with $A_{g_{rx},g_{tx}}(t,f)\Big|_{t=n\Delta t,f=m\Delta f}$~\cite{8424569}.
%
% The~\cref{eq:Wigner} is Wigner Transform~\cite{ronny2017otfs}.
%By applying an SFFT on $Y_{TF}$, we obtain the DD samples,
% \begin{align}
%     \label{eq:SFFT}
%     Y_{DD}[k,l]=\sum_{n=0}^{N-1}\sum_{m=0}^{M-1}Y_{TF}[n,m]e^{-j2\pi\parens*{\frac{kn}{N}-\frac{ml}{M}}}.
% \end{align}
% \textcolor{red}{
% Assuming that the channel can be estimated via the use of pilots, based on \cref{recovery}, $X_{TF}[n,m]$ can be obtained and lead to $X_{DD}[n,m]$ via an SFFT, i.e.,
% \begin{align}
%     \label{eq:SFFT}
%     X_{DD}[k,l]=\sum_{n=0}^{N-1}\sum_{m=0}^{M-1}X_{TF}[n,m]e^{-j2\pi\parens*{\frac{kn}{N}-\frac{ml}{M}}}.
% \end{align}
% *** is this ok?}
% \textcolor{green}{It's mathematically correct. But the receiver won't be able to estimate the $H$ which is in TF domain. The OTFS works in DD domain.}
% \textcolor{red}{The symbols $X_{DD}[k,l]$ can be recovered as follows *****explain}
% \subsection{OTFS Input-Output Relation (I/O)}\label{sec:OTFS_IO}
{
\color{blue}
The received DD domain samples, $y[k,l]$, can be obtained by applying an SFFT on $Y[n,m]$.
It holds that as~\cite{ronny2017otfs}
% {\small
\begin{align}
    y[k,l]
    &= \sum_{n=0}^{N-1}\sum_{m=0}^{M-1}Y[n,m]e^{-j2\pi\parens*{\frac{kn}{N}-\frac{ml}{M}}}, \label{eq:SFFT} \\
    &= \frac{1}{NM}\sum_{k'=0}^{N-1}\sum_{l'=0}^{M-1}x[k',l']h[k-k',l-l'], \label{eq:DDIO_2}\\
    &= \frac{1}{NM} \sum_{k'=0}^{N-1}\sum_{l'=0}^{M-1}x[k-k', l-l']h[k',l']. \label{eq:DDIO}
\end{align}
% }%
% where $h[k,l]$ is the SFFT of $H[n,m]$.
Combining~\cref{eq:DD_spacing,eq:Doppler_spacing,eq:Delay_spacing,eq:TFChannel,eq:SFFT}
{\small
\begin{align}
    h[k', l']
    &= \sum_{n=0}^{N-1}\sum_{m=0}^{M-1} e^{-j2\pi\parens*{\frac{k'n}{N}-\frac{ml'}{M}}} \sum_{j=0}^{J-1} \beta_j \notag\\
    &\times e^{-j2\pi\frac{(k_j+\kappa_j)(l_j+\iota_j)}{NM}}e^{j2\pi\bracks*{(k_j+\kappa_j)\frac{n}{N}-\frac{m}{M}(l_j+\iota_j)}} \label{eq:DDChannel_2}\\
    &= \sum_{j=0}^{J-1}\beta_je^{-j2\pi\frac{(k_j+\kappa_j)(l_j+\iota_j)}{NM}}\mathcal{G}[k',k_j+\kappa_j]\mathcal{F}[l',l_j+\iota_j]. \notag
\end{align}
}%
The $\mathcal{G}[k',k_j+\kappa_j]$ and $\mathcal{F}[l',l_j+\iota_j]$ are in the format of Dirichlet kernel, which is also known as periodic sinc function
\begin{align}
    \mathcal{G}[k',k_j+\kappa_j]
    &\stackrel{\Delta}{=}\sum_{n=0}^{N-1}e^{-j2\pi(k'-(k_j+\kappa_j))\frac{n}{N}}, \label{eq:Doppler_component}\\
    \mathcal{F}[l',l_j+\iota_j]
    &\stackrel{\Delta}{=}\sum_{m=0}^{M-1}e^{j2\pi \frac{m}{M}(l'-(l_j+\iota_j))}. \label{eq:delay_component}
\end{align}
With rectangular window function~\cite{Wei2021}, only one realization of the sinc wave will appear in the DD domain.
For the case of integer Doppler and delay, the DD domain samples will fall on the grid point and~\cref{eq:DDChannel_2} becomes
}%
% Substituting~\cref{eq:DDChannel} into~\cref{eq:DDIO} yields~\cite{raviteja2018otfs}
% {\small
\begin{align}
    h[k',l']
    &=
    \sum_{j=0}^{J-1} \beta_j e^{-j2\pi\frac{k_{j}l_{j}}{NM}} \delta[k'-k_{j}]\delta[l'-l_{j}]. \label{eq:DDChannel} \\
    y[k,l]
    &= \sum_{j=0}^{J-1}\beta_je^{-j2\pi\frac{k_{j}l_{j}}{NM}}x[[k-k_{j}]_N,[l-l_{j}]_M], \label{eq:IO}
\end{align}
% }%
where $[\cdot]_N$ is modular operation with order $N$.

\cref{eq:DDIO_2} can be vectorized as
% {\small
\begin{align}\label{eq:vector_io}
    \mathbf{y}
    =  \mathbf{h}\mathbf{x}+\mathbf{w},
\end{align}
% }%
where $\mathbf{w}\in\C^{NM}$ is noise, $\mathbf{h}\in\C^{NM\times NM}$ is the  channel matrix, and $\mathbf{y}$, $\mathbf{x}$, are DD domain vectorized received symbols and transmitted symbols whose ($l+kM$)-th element is $y[k,l]$ and $x[k,l]$, respectively.
% additive white Gaussian noise (AWGN) with power $\sigma_{\mathbf{w}}^2$.
% $\mathbf{F}_{\textnormal{N}}$ is $N$-point DFT matrix.
% $\mathbf{I}_{\textnormal{N}}$ is $N\times N$ identity matrix representing rectangular pulses and windowing functions.
% $\mathbf{H}_t$ is the time domain channel taking effect in~\cref{eq:received}.
% % $\mathbf{H}_{TF}$ is the matrix representation of~\cref{eq:TFChannel}.
% \textcolor{blue}{
% }
% $\mathbf{H}$ can be estimated with a single pilot~\cite{hong2022delay}, making OTFS more efficient in channel estimation than OFDM ,which requires a full grid of pilots in time-varying channels.
$\mathbf{h}$ can be estimated with a single pilot~\cite{hong2022delay}, and the information-bearing symbols can be estimated via LMMSE equalization.
% is
% \begin{align}\label{eq:lmmse}
%     \tilde{{\mathbf{d}}}
%     =(\mathbf{H}^{\mathsf{H}}\mathbf{H}+\sigma_{\mathbf{w}}^2\mathbf{I})^{-1}\mathbf{H}^{\mathsf{H}}\hat{\mathbf{d}}.
% \end{align}
% Then the symbol can be detected by conventional detectors, \eg correlation detectors, \etc.% \bigskip
% \textcolor{magenta}{**** the following refers to background on OTFS for sensing. Who has proposed the method that you describe in the next 2 lines????  *****}
% \textcolor{red}{Since $H[\cdot,\cdot]$ contains Doppler and delay information of targets, the indices of $h$'s peak can be used to estimate the target's range and velocity.~\cite{9764285,zhang2023radarsensingotfssignaling}}
% \textcolor{blue}{This is addressed in~\cref{eq:DDChannel}}

==> Format.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Packages to Load
%% Text and Math Environment Packages
\RequirePackage{csquotes} %Package to Facilities Quotations
% \RequirePackage[backend=biber, style=ieee, sorting=ynt]{biblatex}
\RequirePackage[english]{babel} %Multilingual Support Must Load the First
% \RequirePackage[utf8]{inputenc} %utf8 Support. Preloaded in Distribution
\RequirePackage[T1]{fontenc} %Better Font Encoding for T1 Type Font
\RequirePackage[shortlabels, inline]{enumitem} %Conflict with Beamer
\RequirePackage[svgnames]{xcolor} %Beamer Has This by Default
\RequirePackage[most]{tcolorbox} %Customized Box. Must Load after xcolor
\RequirePackage{mathtools} %Customize Math Symbols and Theorems
\RequirePackage{amsthm, thmtools, thm-restate} %Better Theorems
% \RiquirePackage{amsmath} %Loaded by mathtools
\RequirePackage{amssymb} %Conflict with Fonts
% \RequirePackage{Fonts} %Must Load after tcolorbox and amsthm
% \let\openbox\undefined %Fix Some Font Issues
\RequirePackage{bm} %Boldface Math, Load after Other Math Font Packages
\RequirePackage{mleftright} %Fixes Some Math Spacing Issues
\RequirePackage{microtype} %Better Font Spacing

%% Table Packages
\RequirePackage{tabularx} %Including Tabular with More Space Option
\RequirePackage{colortbl} %Package to Use Color in Tables
\RequirePackage{multirow} %Package to Use Multirow in Tables
\RequirePackage{multicol} %Package to Use Multicols
\RequirePackage{array} %Math and More Spacing Support in Tables

%% Graphics Packages
\RequirePackage{epstopdf} %Package to Convert eps to pdf in pdfLatex
\RequirePackage{transparent} %Transparent Images
\RequirePackage{graphicx} %Graphics Backend with key-value Arguments
\RequirePackage[export]{adjustbox} %More Arguments for includegraphics
\RequirePackage{subcaption} %Package to Use Subfigure

%% Code Packages
% \RequirePackage{listings} %Loaded by tcolorbox and also no need of minted.
\RequirePackage{algorithm} %Package to Insert Algorithm
\RequirePackage{algpseudocode} %Package to Insert Algorithm

%% Other Packages
\RequirePackage{xspace} %Package to Add Space after Macros
% \RequirePackage{calc} %Package of Calculation in Latex
% \RequirePackage{rotating} %Package to Rotate Objects
% \RequirePackage{pgf, tikz} %Package to Draw Figures.
% \RequirePackage{keyval}
\RequirePackage{orcidlink}
\RequirePackage{hyperref} %Beamer Has This by Default.
\RequirePackage[capitalise]{cleveref} %Must Load after others. Conflict with Beamer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
